Generalizing Pauli Spin Matrices Using Cubic Lattices

In quantum mechanics, the connection between the operator algebraic realization and the logical models of measurement of state observables has long been an open question. In the approach that is presented here, we introduce a new application of the cubic lattice. We claim that the cubic lattice may be faithfully realized as a subset of the self-adjoint space of a von Neumann algebra. Furthermore, we obtain a unitary representation of the symmetry group of the cubic lattice. In so doing, we re-derive the classic quantum gates and gain a description of how they govern a system of qubits of arbitrary cardinality.

==> section3.tex <==
\subsection{The Logic of a Hilbert Lattice}
We are now in a place to relate the importance of $\De$ to a general quantum mechanical system. Let $\mathscr{G}$ be a mechanical system potentially classical or quantum, which will be defined below.  

For expository purposes, we reduce to a classical mechanical system, and then obtain a quantum mechanical system as a generalization. 

A classical mechanical system, $\mathscr{G}(S, O)$ is a set of physical states or physically realizable possibilities for objects in the system, $S$, and a set of observables or physical qualities of interest to the observer of the system, $O$. 
\begin{defin}
The observables of a classical system are real valued Borel measurable functions $f: S \r \R$, and thus an experimentally verifiable question is if $f^{-1}(E) = F$ for some Borel set $F \subseteq S$.
\end{defin}

With implication acting as a partial ordering of the experimentally verifiable statements, and the action of negation, we obtain a logic $L(\mathscr{G}(S,O))$. The logic of the state space is a set of subsets of $S$ and, as defined in \cite{geo}, is then the set of experimentally verifiable questions one can ask of the physical system. To be precise:
\begin{defin}[\cite{geo}]
Let $L$ be a complete lattice with orthocomplementation, $^\perp$, then $L$ is a logic if 
\begin{enumerate}
    \item for any countably infinite sequence $a_1$, $a_2$, \dots of elements of $L$, $\meet_n a_n, \join_n a_n \in L$. 
    \item if $a_1, a_2 \in L$ and $a_1 < a_2$, there exists $b \in L$ such that $b < a_1^\perp$ and $b \join a_1 = a_2$.
\end{enumerate}
\end{defin}

In the classical case and our application, The orthocomplement creates an orthomodular lattice, but this is not the case in full generality. 

In the classical case, the notion of and, $\meet$,  is always defined and commutative, and thus we obtain a Boolean or $\sigma$-finite Boolean algebra when considering the lattice of the logic. However, in a quantum mechanical setting, one does not have perfect knowledge of the state space nor their respective observables, due to the uncertainty principle, which can be seen as a consequence of non-commuting operators. Therefore the issue comes down to the fact that $\meet$ is not always experimentally verifiable. As a consequence, we lose distributivity and retain some form of  ortho-algebraic conditions. Thus, a logic of a quantum mechanical system can be defined as a non distributive mechanical system. In other words, it is the set of experimentally verifiable questions of a system with a natural partial ordering defined by implication and some notion of ortho-complementation.

\begin{defin}
Let $H$ be a Hilbert Space. We define the lattice of closed linear subspaces of $H$ to be the Hilbert Lattice henceforth referred to as $HL$. In this context, $u \join v = span\{u ,v\}$, and $u \meet v = span\{u\} \cap span\{v\}$. For finite dimensional subspaces, the lattice rank coincides with the standard rank. 
\end{defin}

One can directly observe that the Hilbert lattice HL satisfies all the criteria of a logic. Therefore, our choice of embedding space in Theorem \ref{embedding}, has a logical realization. In order to tie things together: the observables are self adjoint linear operators in the von Neumann algebra $B(H)$, and the states $S$ are considered as vector states in $B(H)^\ast$.
\begin{defin} Let $A$ be a Hermitian operator and $ 0 \ne \lambda \in \R$, then $A(\{\lambda\})  = span\{h \in H: Ah = \lambda h\}$, so that $\lambda$ is in the point spectrum of $A$ if $0 < A(\{\lambda\}) \in L(H)$. \cite{geo}
\end{defin}

For compact Hermitian operators we have that the point spectrum gives the full picture, and this is sufficient to describe our general case up to a tolerable approximation error. 
\noindent

\subsection{Merging the implication structures of a Cubic lattice, a Hilbert Lattice, and a von Neumann Algebra}

We now have an order embedding of the poset of ideals of the cubic lattice to the poset of faces of a von Neumann algebra. In particular, all of these maps can be shown to be well defined for addition and multiplication in the von Neumann algebra. Both structures have a fairly diverse set of operations. This section explores how the cubic lattice operations $\meet_C$, $\join_C$, and $\Delta$, the orthomodular Hilbert lattice operations, $\meet_H$, $\join_H$, and $^\perp$, and the von Neumann algebra operations $+$, $\cdot$, and Jordan algebra multiplication,$\circ$, relate. 

The first question is can we lift lattice structure of the lattice of signed sets L(S) to the algebraic structure of the $SA(\M)_+ = (\M, +, \circ)$, where $\M$ is a von Neumann algebra. The answer is partially yes, and utilizes a standard result from logic and computing. 


\noindent We first use a standard result of von Neumann algebras. 
\begin{prop}
The self adjoint operators of von Neumann algebra form an order unit algebra where multiplication is the Jordan product induced by the multiplication of the von Neumann algebra. 
\end{prop}

However, this order unit algebra is not unique to the given von Neumann algebra. There are many possible associative products defining many distinct von Neumann algebras that are consistent with a single underlying Jordan product. For more information, see a discussion of global orientations and Hilbert balls \cite{alfsen}.

We now demonstrate the value of choosing an orthonormal basis. Of course, orthogonal projection operators need not commute even in the finite dimensional case.

\begin{lemma}\label{commuting projections}
Let $H$ be a Hilbert space with an orthonormal basis $\mathscr{B}$. If $F$, $G \subseteq \mathscr{B}$, then $P_FP_G= P_{F \cap G} = P_GP_F$.
\end{lemma}

\begin{proof}
We show the equality for a given element $h \in H$. By definition we have $P_F(h) = \sum_{f \in F} \lan f$ , $h \ran f,\, P_G(h) = \sum_{g \in G} \lan g, h \ran g$, and $P_{F \cap G} = \sum_{f \in F \cap G} \lan f , h \ran f$.
Now, 
\begin{align*}
P_G P_F(h) &= \sum_{g \in G} \lan g , P_F h \ran g \\
&= \sum_{g \in G } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g\\
&= \sum_{g \in  G \cap F } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g + \sum_{g \in G - F } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g
\\
&= \sum_{g \in  G \cap F } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g + \sum_{g \in G - F } \sum_{f \in F} \overline{\lan f, h} \ran \lan g ,  f \ran g \\
&= \sum_{g \in  G \cap F } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g + \sum_{g \in G - F } \sum_{f \in F} \overline{\lan f, h} \ran 0\\
&= \sum_{g \in  G \cap F } \lan g , \sum_{f \in F} \lan f, h \ran f \ran g + 0\\
&=  \sum_{g \in  G \cap F } \lan g ,P_F h \ran g\\
&= \sum_{g \in  G \cap F } \lan P_F g , h \ran g\\
&= \sum_{g \in  G \cap F } \lan g , h \ran g\\
&= P_{F \cap G}(h)
\end{align*}

By symmetry, we have $P_FP_G(h) = P_{F \cap G}(h) = P_G P_F(h)$, and as $h$ was arbitrary, we conclude the result.

% We assume $f \in G$, then for any h \in H, \lan P_G h, f \ran = \lan h, P_G f \ran = \lan h, P_{F \cap G} f \ran  = \lan P_{F \cap G} h , f \ran and by symmetry, \lan P_F h, f \ran = \lan P_{F \cap G }h ,f \ran. 
\end{proof}

\begin{defin}
Let $P$ be the set of projections in $\M^+$ onto a fixed orthonormal basis $\mathscr{B}$. The binary operation XOR denoted by $\oplus: P \times P \r P$ is defined by $A \oplus B = B^\perp A + A^\perp B.$ 
\end{defin}

\noindent We have already discussed that $CL$ can be embedded in $\M$ as a set of projection operators, in particular idempotent operators. Now we have a binary operation from projections onto subsets of a fixed orthonormal basis, $A,B$ defined by $A \join_H B = A \oplus B \oplus AB$ where $\oplus$ is the symmetric addition (XOR) defined above, and $A \meet B = A \circ B$ is the Jordan product. 

\begin{lemma}\label{join and add}
Let $A, B \in B(H)$ be projection operators onto different subsets of the same orthonormal basis of $H$. Then $A \join_{H} B = A + B - A\circ B$, where $+$, $-$ are the standard addition and subtraction induced by the von Neumann algebra. 
\end{lemma}

\begin{proof}
By Lemma \ref{commuting projections}, $AB = A\meet_{H} B = B \meet_{H} A = BA$ by commutativity, and now we can also freely use associativity. Since we are dealing with projection operators, we also have that all operators are idempotent. Now the result follows by a standard computation.
\begin{align*}
A \join_H B &= A \oplus B \oplus AB\\
&= (A \oplus B) \oplus AB\\
&= (A(1-B) + B(1 - A)) \oplus AB\\
 &= (A + B - 2AB) \oplus AB\\
 &= (1 - (A + B - 2AB))(AB) + (1 - AB)(A + B - 2AB)\\
 &= AB - AB - AB + 2AB + A + B - 2AB - AB - AB + 2AB\\
 &= A + B - AB
\end{align*}
\end{proof}
Now we have everything to finish the final major result of the subsection:
\begin{lemma}\label{meet agreement}
For a proper principal lattice filter of the cubic lattice, $F \subseteq CL\subseteq HL$, $\meet_H : F \times F  \r HL = \meet_C : F \times F \r F$.  Equivalently the join of and ideal OL agrees with meet of the Hilbert lattice.
\end{lemma}

\begin{proof}
Let $a, b \in F$. By definition we can write $a$, $b$ as the joins of atoms that are members of the orthonormal basis constructed in Theorem \ref{embedding}, so we can write $a \meet_H b$ in the same orthonormal basis as well. Therefore, we have the same relevant set of atoms for both $HL$ and $CL$ and reduce to this case implicitly for the remainder of the proof.

If $\alpha$ is an atom of $CL\subseteq HL$ such that $\alpha \le a$ and $\alpha \le  b$ then $\alpha \le a \meet_C b$ and $\alpha \le  a \meet_H b$. In addition, these are the only atoms in the commutative Boolean sub-lattice of $HL$ that are less than or equal to $a \meet_C b$ or $a \meet_H b$. By atomisticity of the cubic lattice and the Boolean sub-lattice of the Hilbert lattice,  $a \meet_C b = \join_C\{\a : \alpha \le a \text{ and } \alpha \le b\}$, $a \meet_H b = \join_H\{\a : \alpha \le a \text{ and } \alpha \le b\}$.

As the ordering of $CL$ is inherited from $HL$, $\alpha \join_{H} \beta = inf\{c \in HL: c \ge \alpha, \, c \ge \beta\} \le inf\{c \in CL: c \ge \alpha, \, c \ge \beta\}$. Therefore, $a \meet_H b \le a \meet_C b$. Now by reversing the above argument,  $\alpha \meet_{H} \beta = sup\{c \in HL: c \le \alpha, \, c \le \beta\} \ge sup\{c \in CL: c \ge \alpha, \, c \ge \beta\}$, and $a \meet_H b \ge a \meet_C b$. 
\end{proof}

\begin{remark}
The subtle and key part of this proof is that one does not lose atoms when finding lattice meets in the cubic lattice i.e. all atoms that are contained in both subfaces remain. However, when we consider joins of two subfaces, one gains atoms that were in neither subface. One can also not substitute the argument with co-atomisiticity as the set of co-atoms of $HL$ and $CL$ are not the same. In the finite dimensional case, one can view that the intersection of two subfaces contains all common lower dimensional subfaces, but the next largest subface containing both may include additional vertices. 
\end{remark}

\begin{theorem}\label{cubic meet and product}
For a principal lattice filter of the cubic lattice, $F \subseteq CL\subseteq HL$, $\meet_C : F \times F \r F$ is equal to the Jordan product and associative product of $B(H)$. 
\end{theorem}


\begin{proof}
The theorem follows as a result of Lemma \ref{commuting projections} and Lemma \ref{meet agreement}.
\end{proof}

% \begin{proof}
% We know from \cite{oliveira} that for a given filter, $F$ in $C$, the lattice $(F, \join, \meet)$ forms a Boolean algebra, so now we use the above propositions to both embed the Boolean algebra in $\M$, and immediately conclude that the ring $(R, +, \circ)$, where  $A \join B :=  A + B - AB$,  and $\circ$ is the Jordan product multiplication in the order unit algebra. 
% \end{proof}

In many standard arguments, XOR is taken to be addition modulus 2, so we present the explicit computations for demonstrating that distributivity of the ring is equivalent to distributivity in the Boolean algebra.

\begin{lemma}\label{distributivity equilvalence}
Let $\mathscr{B}$ be an orthonormal basis of a Hilbert space $H$ and $A, B, C$ be projections onto subsets of $ \mathscr{B}$. 
\begin{enumerate}[(1)]
\item $\meet_H$ distributivity and multiplicative distributivity are equivalent.
\item $\join_H$ distributivity and XOR distributivity are equivalent.
\end{enumerate}
\end{lemma}

\begin{proof}
We first demonstrate the $\meet_H$ distributivity and multiplicative distributivity are equivalent using Lemma \ref{join and add}:
 \begin{align*}
A \meet_H (B \join_H C) &= A  (B + C - BC) \\
&= AB + AC - ABC\\
&= (A \meet_H B) \join_H (A \meet_H C)
\end{align*}

In order to prove (2), we first use a simplification that $A \oplus B  = (A \join_H B) - (A \meet_H B)$:
\begin{align*}
A \oplus B &= AB^\perp + BA^\perp\\
&= A(1 - B) + B(1-A)\\
&= A - AB + B - AB\\
&= (A + B - AB) - AB\\
&= (A \join_H B) - (A \meet_H B).
\end{align*}
Then, 
\begin{align*}
A \oplus (BC) &= (A \join_H (B \meet_H C)) - (A \meet_H (B \meet_H C))\\
&= ((A \meet_H B) \join_H (A \meet_H C)) - (A \meet_H B \meet_H C)\\
&= (A \meet_H B) \oplus (A \meet_H C)\\
&= (AB) \oplus (AC).
\end{align*}

\end{proof}

% Lastly, the equivalency of the filters of CL, and the ideals of OL when considered as rings as opposed to just posets follows from Theorem  \ref{antiismorphism}.
% We use a standard result:
% \begin{lemma}\label{Boolean ring and lattice}
% Every Boolean algebra is a Boolean ring with unity with respect to the symmetric addition and multiplication, which coincides with the Jordan product for commutative von Neumann (sub) algebras.
% \end{lemma}

\begin{theorem}\label{Boolean Hilbert sub lattice}
The lattice of projections onto subsets of a fixed orthonormal basis, $L(\join_H, \meet_H)$, form a Boolean algebra. 
\end{theorem}

\begin{proof}
By \ref{commuting projections}, we have shown $L$ when considered as ring $L(\oplus, \cdot)$ is firstly closed under $\cdot$, and secondly commutative. A ring of commutative  idempotents is Boolean, so $L$ is a Boolean ring. Then $L$ is distributive as a ring, so we have $L$ is distributive as a lattice by Lemma \ref{distributivity equilvalence}. As $L$ is an orthomodular sublattice of $HL$, we have that $L$  is a Boolean algebra by \cite{qlog1}.
\end{proof}

Theorem \ref{cubic meet and product} demonstrates that the cubic lattice and the Hilbert lattice share a common meet described by the product of a von Neumann algebra. However the join structure of the lattices is very different. One can view this as a different question asked of the system. The join of two observables in a Hilbert lattice asks the minimum subspace where all events are observable. The join of two observables in a cubic lattice asks for the minimum subspace where both observables are entangled. 

Theorem \ref{Boolean Hilbert sub lattice} shows a Boolean algebra containing the cubic lattice when embedded as in Theorem \ref{embedding}. However, the Boolean complement is order reversing and inherently irreconcilable with the unitary propagation of a quantum system. In addition, the Boolean structure is in a sense too rigid  and well defined to fully encode the entanglement of a quantum system as stipulated by requirements in \cite{qlog2}:
\begin{enumerate}
    \item Completeness
    \item Atomicity
    \item Superposition principle: (atom $c$ is a superposition of atoms $a$ and $b$ if $c \ne a$, $c \ne b$, and $c \le a \join b.$)
    \begin{enumerate}
        \item Given two different atoms $a$ and $b$, there is at least one other atom $c$ that is a superposition of $a$ and $b$.
        \item If the atom $c$ is a superposition of the distinct atoms $a$ and $b$, then $a$ is a superposition of $b$ and $c$.
    \end{enumerate}
    \item Unitary Operators: Given any two orthogonal atoms $a$ and $b$ in $HL$, there is a unitary operator $U$ such that $U(a) = b$. 
    \item Infinite Orthogonality: $HL$ contains a countably infinite sequence of orthogonal elements. 
\end{enumerate}

One can see that the Hilbert lattice satisfies these criteria while the Boolean lattice defined above fails the the superposition principle. The following subsection discusses a notion of order preserving complementation of cubic lattice and its Boolean subalgebras.



\subsection{A Unitary Negation}
Of course one's interest in physical systems involves more than their states and their experimentally verifiable questions. One also wants to know how a state changes over time based on its current state up to one's ability to observe the state experimentally. In the classical setting, if one observes the states of the system at a time, $t_0$, and we have perfect knowledge of some dynamic law $U(t)$ of the system, then we can predict the states of the system at time $t_0 + t.$ However, in a quantum mechanical system, we will not have such predictive power, but we still have a dynamic law $U(t)$ represented by a unitary operator as discussed in the axiomitization of quantum mechanics stated in section 1. 

A major issue that immediately occurs is that the notion of orthocomplementation of the logic is order reversing, while unitary operators are order preserving. Therefore, these two structures, which are necessary for the understanding of a quantum mechanical system, are, at some level, irreconcilable. We have discussed in the previous subsection that our embedding space is consistent with the modern literature. Now we will show that $\De$ when represented as a unitary operator may help bridge the gap to a unitary negation in some sense. 

As we have discussed the basic operations $\meet$ and $\join$ in the respective lattices, we want to discuss the relation between the remaining operations: $^\perp$ and $\De$. We first need to introduce some additional definitions. For additional context, see \cite{alfsen}.

\begin{defin}
A symmetry in a von Neumann algebra is a Hermitian involution. An e-symmetry in a von Neumann algebra is a Hermitian element $s$ such that $s^2 = e$, where $e$ is an orthogonal projection. When the specific projection $e$ is not relevant, we will just say partial symmetry \cite{alfsen}.  
\end{defin}

\begin{defin}
A projection in a von Neumann algebra is halvable if it is the sum of two Murray-von Neumann equivalent projections. 
\end{defin}

\begin{defin}
A partial symmetry $s$ in a von Neumann algebra $\M$ will be called balanced if it has a canonical decomposition $s = p - q$, and $p \sim q$ where $\sim$ denotes Murray-von Neumann equivalence. \cite{alfsen}
\end{defin}

\begin{prop}[Proposition 7.7 \cite{alfsen}]\label{halvable equivalence}
If $e$ is a projection in a von Neumann algebra $\M$, then the following are equivalent:
\begin{enumerate}[i)]
    \item $e$ is halvable
    \item there exists a Jordan orthogonal pair of $e$-symmetries
    \item there exists a balanced e-symmetry. 
\end{enumerate}
\end{prop}

\begin{theorem}
There exists a unitary representation of $Aut(L(S))$ on $B(H)$ where $H$ is constructed in Theorem \ref{embedding}.
\end{theorem}

\begin{proof}
As the Hilbert lattice is a atomic and atomistic lattice, and the atoms $CL$ form an orthonormal basis of $H$, an automorphism on the atoms of $CL$ defines a permutation of the atoms of $HL$. Therefore, lattice automorphism of $CL$ embed into the permutation group in $B(H)$, in particular they are unitary. 
\end{proof}

Note that in the original representation of automorphisms of CL are reflections of the half plane or permutations of a basis of size $|S|$, specifically the representations are embedded in the orthogonal group. One can view this difference as choice in matrix representation. 

\begin{prop}\label{unitary involution}
An involution $U$ in a von Neumann algebra is Hermitian if and only if $U$ is unitary.
\end{prop}

\begin{proof}
Let $U \in B(H)$ involution.
Suppose $U$ is unitary, then 
\begin{align*}
U^2 &= I\\
U^\ast U^2 &= U^\ast\\
(U^\ast U)U &= U^\ast\\
U &= U^\ast
\end{align*}

If $U$ is Hermitian, then for any $h \in H$
\begin{align*}
\lan U^2 h , h \ran &= \lan h ,  h \ran\\
\lan U h , U^\ast h \ran &= \lan h ,  h \ran\\
\lan U h , U h \ran &= \lan h ,  h \ran\\
||Uh|| &= ||h||
\end{align*}
Therefore, $U$ is an isometry, and as $U^2 = I$ is surjective, so $U$ must be as well. 
\end{proof}

\begin{coro}
The unitary representation of $\Delta$, $U_\De$ on $B(H)$ is a symmetry. 
\end{coro}

\begin{proof}
$\Delta$ is an involution by definition, so the result follows from the above arguments.
\end{proof}

As a symmetry, we have the a canonical decomposition of $U_\De = \frac{1 + U_\De}{2} - \frac{1 - U_\De}{2}$, where $\frac{1 + U_\De}{2}$ and $\frac{1 - U_\De}{2}$ are orthogonal projection operators.


\begin{prop}
The symmetry $U_\Delta$ is a balanced symmetry of $B(H)$.
\end{prop}

\begin{proof}
We need only consider coatoms of $c, \Delta(c) \in CL$ with associated projections $p_c$, $p_\Delta(c)$, and let $U_\Delta$ be the unitary representation of $\Delta$. Then we have the action of the unitary symmetry $U_\Delta p_c U_\Delta = p_{\Delta(c)}$. Now let $s = p_c - p_{\Delta(c)}$. Then,
\begin{align*}
    U_\Delta s U_\Delta &= U_\Delta(p_c - p_{\Delta(c)}) U_\Delta\\
    &= p_{\Delta(c)} - p_c \\
    &= -s
\end{align*}

Therefore,
\begin{align*}
U_\Delta s &= U_\Delta s U_\Delta^2\\
&=( U_\Delta s U_\Delta)U_\De\\
&= -sU_\Delta.
\end{align*}
The result follows by \ref{halvable equivalence}. Explicitly the symmetry similarity transformation, $s$, takes $\dfrac{1 + U_\De}{2}$ to $\dfrac{1 - U_\De}{2}$, and unitary similarity implies Murray-von Neumann equivalence.
\end{proof}

Of course the choice of coatom was arbitrary in the above proof, so we have the following slightly more general result. 

\begin{coro}\label{pauli constuction}
For any given coatom $c \in CL$, the symmetry $s = p_c - p_{\Delta(c)}$ anticommutes with $U_\Delta$. 
\end{coro}


\begin{theorem}\label{Delta and perp agreement}
The action of $^\perp$ on $HL$ on the coatoms of $CL$ is a symmetry and coincides element-wise with the unitary symmetry associated with $\Delta$.
\end{theorem}

\begin{proof}
The result follows as for all $c \in CL$, $p_c^\perp = 1 - p_c = p_{\Delta(c)} = U_\Delta p_c U_\Delta$. 
\end{proof}


\begin{coro}
Let $c$, $\Delta(c) \in CL$ be coatoms, then the lattice operations of $CL$ and $HL$ coincide. 
\end{coro}

\begin{proof}
Consider $c, \Delta(c) \in CL$ and the associated projection operators $p_c$ and $p_{\Delta(c)}$, which project on a generalized simple tensor $u$ of the form $u_i = V_i$ for all $i \in I -\{j\}$ and for exactly one $j \in I$, $u_j = v$, $v \in V_j$. 
By lemma \ref{meet agreement}, we need only show that $p_c \join_{H} p_{\Delta(c)} =  p_c \join_{C} p_{\Delta(c)}$. Further, we reduce to showing $p_c \join_{H} p_{\Delta(c)} \ge p_c \join_{C} p_{\Delta(c)}$ by the argument in the proof of Lemma \ref{meet agreement}. 

Now by Theorem \ref{Delta and perp agreement}, $p_c^\perp = p_{\Delta c}$, so $p_{c} \join_H p_{\Delta c} = p_c + p_{\Delta c} = 1 \ge p_{\De  c} \join_C p_c$, where orthogonality is implicitly used in the first set of equalities. 
\end{proof}

\begin{exmp}
Let $H = \Co^2$, and $U_\De, s$ be constructed as above for the standard basis. 
\begin{align*}
U_\De &= \begin{bmatrix}
0 & 1 \\
1 & 0
\end{bmatrix},\\
s &= \begin{bmatrix}
1 & 0 \\
0 & -1
\end{bmatrix}, \\
iU_\De s &= 
\begin{bmatrix}
0 & -i\\
i & 0
\end{bmatrix}
\end{align*}
We recognize these matrices as the famous Pauli matrices!
\end{exmp}

\begin{coro}
The operators of Corollary \ref{pauli constuction} give an explicit construction for the generalization of Pauli matrices to a cubit system up to arbitrary cardinality, $\omega$. Furthermore, as a computational device, we can use our original lower dimensional matrix representation to perform these matrix computations on a $O(\omega)$ vector space as opposed to the exponentially larger $O(2^\omega)$ vector space used in the standard construction. 
\end{coro}

We now have an order preserving lattice isomorphism of $HL$, $U_\Delta$, and an order reversing lattice anti-isomorphism, $^\perp$, that agree on certain subset specifically the coatoms of $CL$. Furthermore, we have that for pairs of coatoms which half the identity, we have that the canonical symmetry associated with the pair anti-commutes with the action $U_\Delta$, and therefore the action of $^\perp$ when we consider the action element wise. However, $U_\Delta$ is distributive on the difference of the projections while $^\perp$ is not except on a principle filter. In essence, we now have a linear distributive operation that agrees element-wise with $^\perp$ on the coatoms of $CL$. 

As we move forward, this relationship will become more relevant. The lattice automorphisms of $CL$, permutations of coatoms of $CL$ that commute with $\Delta$, and the commutant of $\Delta$ are all intimately related in a way that will be discussed. The above section shows that in some sense this relationship holds with $^\perp$ on the Hilbert lattice as well and the reader should keep this in mind.
% \newpage

